When the Critic Falls Behind: Co-Evolving Rubrics and Harnesses for Continual Agent Self-Improvement

Autonomous agents increasingly depend on harnesses that govern interaction, memory, tools, and execution around large language models (LLMs). While recent work has begun to evolve these harnesses from execution experience, the supervision used to guide evolution often remains relatively static, making it difficult to track changing behavioral weaknesses across rounds and potentially limiting generalization to unseen tasks. To address this issue, we propose RuHarness, a rubric--harness co-evolution framework for continual agent self-improvement. RuHarness continually discovers and reassesses behavioral criteria from execution trajectories, prioritizes the most relevant unresolved weaknesses, and uses them to guide targeted harness updates while keeping the task objective fixed. Extensive experiments across diverse agent tasks and backbone models show that RuHarness outperforms strong harness-evolution baselines, particularly on unseen held-out tasks. Further analyses show that adaptive rubric prioritization tracks shifting weaknesses and supports more sustained improvement and stable generalization across evolution rounds.

==> figure/Prompt/7_harness_candidate_review.tex <==
\begin{tcblisting}{
    breakable,
    width=\columnwidth,
    title=\textbf{Harness Candidate Review},
    colback=gray!5,
    colframe=black,
    colbacktitle=gray!10,
    coltitle=black,
    arc=1mm,
    boxrule=1pt,
    boxsep=0pt,
    left=2mm,
    right=2mm,
    top=2mm,
    bottom=2mm,
    before skip=4pt,
    after skip=4pt,
    toptitle=1.5mm,
    bottomtitle=1.5mm,
    listing only,
    listing options={
        basicstyle=\ttfamily\footnotesize,
        breaklines=true,
        breakautoindent=false,
        breakindent=0pt,
        columns=fullflexible,
        keepspaces=true,
        showstringspaces=false
    }
}
You are reviewing a proposed change to an agent's harness BEFORE it is evaluated. Approve it or reject it. Do not rewrite it, do not suggest an alternative, and do not predict a benchmark score - none of those are your job, and a rewrite here would be evaluation of a change nobody planned.

THE PLAN:

Hypothesis:
{hypothesis}

Target criteria:
{criteria_list}

Evidence cited:
{evidence_text}

Expected observable change:
{expected_behavior}

Risks the planner identified:
{risks}

Component roles:
{roles_text}

THE ACTUAL EDITS, as they will be applied:
{edits_text}

Reject the change if ANY of these is true:

1. The edits do not follow from the stated evidence - they are generic "be more careful" advice attached to a specific diagnosis.

2. A component's edit contradicts its assigned role, or duplicates another component's edit so that two components now say the same thing.

3. The change invents a capability the component does not have.

4. The change creates an obstacle the agent must then work around: control text passed to an external system that cannot interpret it, a rule that blocks calls the agent depends on, or a policy that conflicts with another policy in the same bundle.

5. An edit aims at the wrong polarity - it would make the criterion "violated" more likely rather than "satisfied".

Approve if none of those hold. Approving a mediocre-but-coherent change is correct; rejecting everything leaves the round with no arms and no information, which is worse.

Output ONLY a single JSON object:
{
  "approved": true | false,
  "reason": "<one sentence; if rejecting, name which numbered condition>"
}

Do not include any other text - no markdown, no commentary. Just the JSON.
\end{tcblisting}
\vspace{6pt}
\captionof{figure}{Prompt template for harness candidate review.}
\label{fig:harness candidate review}
